Noncoherent MIMO Communications: Theoretical Foundation, Design Approaches, and Future Challenges

Noncoherent communication is a promising paradigm for future wireless systems where acquiring accurate channel state information (CSI) is challenging or infeasible. It provides methods to bypass the need for explicit channel estimation in practical scenarios such as high-mobility networks, massive distributed antenna arrays, energy-constrained Internet-of-Things devices, and unstructured propagation environments. This survey provides a comprehensive overview of noncoherent communication strategies in multiple-input multiple-output (MIMO) systems, focusing on recent advances since the early 2000s. We classify noncoherent communication schemes into three main approaches where CSI-free signal recovery is based on subspace detection (i.e., Grassmannian signaling), differential detection, and energy detection, respectively. For each approach, we review the theoretical foundation and design methodologies. We also provide comparative insights into their suitability across different channel models and system constraints, highlighting application scenarios where noncoherent methods offer performance and scalability advantages over traditional coherent communication. Furthermore, we discuss practical considerations of noncoherent communication, including compatibility with orthogonal frequency division multiplexing (OFDM), resilience to hardware impairments, and scalability with the number of users. Finally, we provide an outlook on future challenges and research directions in designing robust and efficient noncoherent systems for next-generation wireless networks.

==> acronyms.tex <==
\usepackage[toc,acronym,nonumberlist,nopostdot]{glossaries}

\makeatletter
%% patch first occurence of "\@gls@link[#1]{#2}{\@glo@text}", as this is the one for \glsused{#2}
\patchcmd{\@gls@}
  {\@gls@link[#1]{#2}{\@glo@text}}
  {\@gls@link[#1,hyper=false]{#2}{\@glo@text}}
  {}{}

  \patchcmd{\@glspl@}
  {\@gls@link[#1]{#2}{\@glo@text}}
  {\@gls@link[#1,hyper=false]{#2}{\@glo@text}}
  {}{}

  \patchcmd{\@Gls@}
  {\@gls@link[#1]{#2}}
  {\@gls@link[#1,hyper=false]{#2}}
  {}{}

\patchcmd{\@GLS@}
  {\@gls@link[#1]{#2}{\MakeUppercase{\@glo@text}}}
  {\@gls@link[#1,hyper=false]{#2}{\MakeUppercase{\@glo@text}}}
  {}{}
\makeatother

\newacronym{AWGN}{AWGN}{additive white Gaussian noise}
\newacronym{iid}{i.i.d.}{independent and identically distributed}

\newacronym{MIMO}{MIMO}{multiple-input multiple-output}
\newacronym{SIMO}{SIMO}{single-input multiple-output}
\newacronym{MISO}{MISO}{multiple-input single-output}
\newacronym{SISO}{SISO}{single-input single-output}

\newacronym{PMF}{PMF}{probability mass function}

\newacronym{CSI}{CSI}{channel state information}
\newacronym{SNR}{SNR}{signal-to-noise ratio}
\newacronym{DoF}{DoF}{degrees of freedom}
\newacronym{BC}{BC}{broadcast channel}
\newacronym{MAC}{MAC}{multiple-access channel}
\newacronym{SER}{SER}{symbol error rate}
\newacronym{BER}{BER}{bit error rate}
\newacronym{PEP}{PEP}{pairwise error probability}

\newacronym{USTM}{USTM}{unitary space-time modulation}
\newacronym{BSTM}{BSTM}{Beta-variate space-time modulation}

\newacronym{KL}{KL}{Kullback–Leibler}

\newacronym{IoT}{IoT}{Internet of Things}
\newacronym{IIoT}{IIoT}{Industrial Internet of Things}
\newacronym{mMTC}{mMTC}{massive machine-type communication}
\newacronym{URLLC}{URLLC}{ultra-reliable low-latency communication}
\newacronym{HRLLC}{HRLLC}{hyper-reliable low-latency communications}
\newacronym{UAVs}{UAVs}{unmaned aerial vehicles}

\newacronym{PAM}{PAM}{unipolar pulse amplitude modulation}
\newacronym{ASK}{ASK}{amplitude shift keying}
\newacronym{QAM}{QAM}{quadrature amplitude modulation}
\newacronym{PSK}{PSK}{phase shift keying}
\newacronym{DPSK}{DPSK}{differential phase shift keying}
\newacronym{DBPSK}{DBPSK}{differential binary phase shift keying}
\newacronym{DQPSK}{DQPSK}{differential quadrature phase shift keying}
\newacronym{DSSS}{DSSS}{direct sequence spread spectrum}
\newacronym{AP}{AP}{alternating projection}

\newacronym{CDF}{CDF}{cumulative distribution function}
\newacronym{ML}{ML}{maximum likelihood}
\newacronym{mmWave}{mmWave}{milimeter-wave}
\newacronym{5G}{5G}{the fifth generation}
\newacronym{6G}{6G}{the sixth generation}
\newacronym{BS}{BS}{base station}
\newacronym{OTA}{OTA}{over-the-air}
\newacronym{LTE}{LTE}{long term evolution}
\newacronym{OFDM}{OFDM}{orthogonal frequency division multiplexing}
\newacronym{DL}{DL}{deep learning}
\newacronym{THz}{THz}{terahertz}
\newacronym{QEC}{QEC}{quantum error correction}
\newacronym{CFO}{CFO}{carrier frequency offset}
\newacronym{IQI}{IQI}{I/Q imbalance}

\newacronym{RIS}{RIS}{reconfigurable intelligent surface}
\newacronym{ISAC}{ISAC}{integrated sensing and communication}
\newacronym{UMA}{UMA}{unsourced multiple access}
\newacronym{HWI}{HWI}{hardware impairment}
\newacronym{OTFS}{OTFS}{orthogonal time frequency space}
\newacronym{LPD}{LPD}{low probability of detection}
\newacronym{DC}{DC}{direct current}
%\newacronym{RIS}{RIS}{reconfigurable intelligent surface}
\newacronym{STBC}{STBC}{space-time block code}
